The Disjunction-Free Fragment of D2 is Three-Valued

In this article, the disjunction-free fragment of Ja\'skowski's discussive logic D2 in the language of classical logic is shown to be complete with respect to three- and four-valued semantics. As a byproduct, a rather simple axiomatization of the disjunction-free fragment of D2 is obtained. Some implications of this result are also discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{257}
\providecommand{\publicationstatus}{A. Indrzejczak, M. Zawidzki (Eds.): Non-Classical Logics.\\ Theory and Applications (NCL'24).\\
EPTCS 415, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.415.22}{10.4204/EPTCS.415.22}}

